DADA: Dialect Adaptation via Dynamic Aggregation of Linguistic Rules

Existing large language models (LLMs) that mainly focus on Standard American English (SAE) often lead to significantly worse performance when being applied to other English dialects. While existing mitigations tackle discrepancies for individual target dialects, they assume access to high-accuracy dialect identification systems. The boundaries between dialects are inherently flexible, making it difficult to categorize language into discrete predefined categories. In this paper, we propose DADA (Dialect Adaptation via Dynamic Aggregation), a modular approach to imbue SAE-trained models with multi-dialectal robustness by composing adapters which handle specific linguistic features. The compositional architecture of DADA allows for both targeted adaptation to specific dialect variants and simultaneous adaptation to various dialects. We show that DADA is effective for both single task and instruction finetuned language models, offering an extensible and interpretable framework for adapting existing LLMs to different English dialects.

==> sections/not-used.tex <==
% \begin{table*}[!ht]
%     \centering
%     \resizebox{0.75\textwidth}{!}{%
%     \begin{tabular}{ccccc|cccccccc}
%         \multicolumn{5}{c|}{Dialect Adaptation Details} & \multicolumn{2}{c}{Test Performance} \\ \hline
%         Backbone & Method & Data & Total Params. & Dialect Params. & \AAVE{} & \SAE{}\\ \hline
%         \multirow{2}{*}{\textit{pretrained}} & Finetuning & \SAE{} & $125 M$ & $0$ & 83.4 & 86.2 \\
%          % & Finetuning & AAVE & $125 M$ & $125 M$ & ~ & ~ \\
%          & Finetuning & \SAE{} + \AAVE{} & $125 M$ & $125 M$ & 84.8 & 85.6 \\\hdashline
%         \multirow{3}{*}{\textit{SAE finetuned}} & Finetuning & \AAVE{} & $125 M$ & $125 M$ & 86.2 & 87.4 \\
%         & Adapter & \AAVE{} & $126 M$ & $1.5 M$ & 86.1 & 87.4 \\
%         & \oursShort{} & \AAVE{} & $155 M$ & $30.8 M$ & 86.6\best{} & 87.6 \best{} \\
%     \end{tabular}}
%     \caption{\textbf{\AAVE{} Adaptation} results of \texttt{RoBERTa Base} \cite{roberta}. \textit{pretrained} denotes the pretrained \texttt{RoBERTa Base} model, while  \textit{SAE finetuned} denotes the \texttt{RoBERTa Base} model that has been finetuned on the original \SAE{} MNLI dataset. \oursShort{} demonstrates superior performance on \AAVE{} and \SAE{} compared to all other methods evaluated (marked as \best{}).}
%     \label{tab:aave_results}
% \end{table*}






% \subsection{Pronouns}
% There are 47 pronoun features in eWAVE, and they cover 39 of them (83\%). While simple regular expressions can cover some pronoun mappings, this is not always possible since English maps the same surface forms to different grammatical roles.\footnote{For example, \textit{her} is both the accusative in ``give it to her`` and the noun modifier in ``her cart,'' while the masculine pronouns in ``give it to him'' and ``his cart'' differ. This problem was observed but not solved in the rule-based perturbation augmentation of \citet{qian2022perturbation}.} They overcome this problem by conditioning rules on pronouns' syntactic roles.
% %in a dependency parse. %(f10)
% They also condition on coreference for referential pronouns [\ewave{29}], and on verb frames to identify benefactive datives [\ewave{9}]. Furthermore, they swap the morphology of possession [\ewave{20}],
% %,\footnote{e.g., \textit{his book} $\rightarrow$ \textit{he book} [20]} number,\footnote{e.g., \textit{}} 
% %and grammatical function [\ewave{}],
% %\footnote{e.g., \textit{}} 
% change reflexive marking [\ewave{11}-\ewave{16}], swap animate pronouns for inanimate objects [\ewave{1}-\ewave{2}],
% %\footnote{e.g., \textit{it's a good bike} $\rightarrow$ \textit{she's a good bike} [1]} 
% and include additional elements like reduplication [\ewave{40}]. In summary, their pronoun perturbation rules %, like all \mval{} transformations
% account for linguistic structure and are not merely surface manipulations.

% \subsection{Noun Phrases}
% Among their 31 noun phrase perturbations, they 
% %make extensive use of \texttt{spaCy} as well as noun inflection resources to 
% regularize or modify plural morphology [\ewave{49}]
% %\footnote{e.g., \textit{wives} $\rightarrow$ \textit{wifes} [49]} 
% and comparison strategies [\ewave{80}],
% %\footnote{e.g., \textit{prettiest sunset} $\rightarrow$ \textit{most pretty sunset} [80]} 
% to drop or modify articles [\ewave{60}],
% %\footnote{e.g., \textit{She's got a toothache} $\rightarrow$\textit{She's got the toothache} [60]} % indicate how many features here
% construct phrases for possession [\ewave{75}],
% %\footnote{e.g., \textit{he was my sister's husband} $\rightarrow$ \textit{he was for my sister husband} [75]} 
% and adjust the tree adjoining order to create adjective postfixes [\ewave{87}].
% %\footnote{e.g., \textit{the Eastern or Western part} $\rightarrow$ \textit{the part Eastern or Western} [87]}

% \subsection{Tense and Aspect} 
% Tense and aspect perturbations include alternative inflections and auxiliaries to mark tense [\ewave{117}],
% %\footnote{e.g., \textit{I will be leaving} $\rightarrow$ \textit{I leaving} [117]} 
% including immediate vs. distant future [\ewave{119}],
% %\footnote{e.g., \textit{I will do it} $\rightarrow$ \textit{I would do it} [119]} 
% as well as perfect aspect [\ewave{99}].
% %\footnote{e.g., \textit{I've eaten} $\rightarrow$ \textit{I ate} [99]} 
% %insert perfect auxiliary markers,\footnote{e.g., \textit{She already read} $\rightarrow$ \textit{She slam read} [107]},

% \subsection{Mood}
% \mval{} includes perturbations that inject double modals [\ewave{121}]
% %\footnote{e.g., \textit{We could do that} $\rightarrow$ \textit{We might could do that} [121]} 
% and quasi-modals [\ewave{126}],
% %\footnote{e.g., \textit{They're about to leave} $\rightarrow$ \textit{They're finna leave} [126]} 
% change verb inflections under modal scope [\ewave{123}],
% %\footnote{e.g., \textit{I wish I could get it} $\rightarrow$ \textit{I wish I can get it} [123]}, 
% and introduce auxiliaries to mark the sequential or irrealis mood [\ewave{106}].
% %\footnote{e.g., \textit{If you tell them, they'll imprison you} $\rightarrow$ \textit{If you tell them, they be done imprison you} [106]}

% \subsection{Verb Morphology}
% Verb morphology features include levelling certain finite and non-finite verb forms [\ewave{130}]
% %\footnote{e.g., \textit{He had gone} $\rightarrow$ \textit{He had went} [130]}, 
% adding suffixes for transitive verbs [\ewave{143}],
% %\footnote{e.g., \textit{You can see the fish} $\rightarrow$ \textit{You can see 'im fish} [143]}, 
% and building \textit{serial verb phrases} \citep{tallerman2019understanding} to mark passive constructions [\ewave{153}],
% %\footnote{e.g., \textit{John was scolded by his boss} $\rightarrow$ \textit{John give his boss scold} [153]}
% indirect objects [\ewave{148}],
% %\footnote{e.g., \textit{I bought rice for you} $\rightarrow$ \textit{I bought rice give you} [148]} 
% or the movement of direct objects [\ewave{150}].

% \subsection{Negation}
% \mval{} includes rules for building phrases with negative concord [\ewave{154}],
% %\footnote{e.g., \textit{I don't want any help} $\rightarrow$ \textit{I don't want no help} [154]} 
% and forms of negation with the negation words \textit{never}, \textit{no}, \textit{not}, \textit{no more} or \textit{ain't}, as well as special invariant tags for questions [\ewave{166}].

% \subsection{Agreement}
% They implement the invariant present tense [\ewave{170}], the existential dummy \textit{it} [\ewave{173}].

% \subsection{Relativization}
% These perturbations modify the form of the relativizer [\ewave{186}-\ewave{190}], as well as drop [\ewave{193}] or introduce new shadow pronouns [\ewave{194}], such as double relativizers [\ewave{191}] and phrasal forms [\ewave{192}]. Their perturbations also operate on the sentence structure by forming correlative constructions [\ewave{196}], deleting stranded prepositions [\ewave{198}], and moving the relative clause before the head noun [\ewave{199}].

% \subsection{Complementation}
% These perturbations can change the form of the complementizer [\ewave{200}, \ewave{201}], delete [\ewave{208}, \ewave{209}] or introduce additional complementizer words [\ewave{203}, \ewave{204}], build existential constructions from complementizer phrases [\ewave{205}, \ewave{206}], and modify the verb in the non-finite clause complement [\ewave{210}].

% \subsection{Adverbial Subordination}
% Their perturbation rules introduce clause-final conjunctions [\ewave{211}, \ewave{212}] and double conjuctions [\ewave{214}, \ewave{215}], and remove the adverb in verb-chaining constructions [\ewave{213}], which together represent the five adverbial subordination features in eWAVE.

% \subsection{Adverbial Prepositions}
% In this section, they drop prepositions [\ewave{216}] and replace adverbs with their adjectival forms [\ewave{220}, \ewave{221}]. 
% %(e.g., \textit{she speaks softly} $\rightarrow$ \textit{she speaks soft}). 
% They also include the word \textit{too} as a qualifier [\ewave{222}].

% \subsection{Discourse and Word Order}
% In discourse, they insert the word \textit{like} as a focus [\ewave{234}] or quotation marker [\ewave{235}]. Their phrase-based perturbations include fronting and clefting [\ewave{223}, \ewave{224}], subject–auxiliary inversion in both negation phrases [\ewave{226}] and indirect questions [\ewave{227}], and a lack of inversion in certain questions [\ewave{228}, \ewave{229}]. These rules significantly alter the sentence structure, and in this way radically differ from prior token-level data augmentation techniques like synonym replacement \citep{wei-zou-2019-eda}. Their approach here is most similar to \textit{constituency replacement} \citep{sutiono2022syntax}.

% \begin{table*}
% \centering
% \resizebox{0.8\textwidth}{!}{%
% \def\arraystretch{1.15}
% \begin{tabular}{lrrrrl}
% \toprule
% \textsc{Abbr} & \textsc{\# Feat.} & \textsc{\% Feat.} & \textsc{\# Val.} & \textsc{\% Val.} & \textsc{Dialect} \\ \midrule
% AborE&89&83.2\%&57&53.3\%&Aboriginal English\\\hline
% AppE&65&85.5\%&51&67.1\%&Appalachian English\\\hline
% AusE&54&90.0\%&40&66.7\%&Australian English\\\hline
% AusVE&47&83.9\%&34&60.7\%&Australian Vernacular English\\\hline
% BahE&107&83.6\%&70&54.7\%&Bahamian English\\\hline
% BlSAfE&95&88.0\%&71&65.7\%&Black South African English\\\hline
% CamE&76&87.4\%&62&71.3\%&Cameroon English\\\hline
% CFE&49&90.7\%&39&72.2\%&Cape Flats English\\\hline
% ChIsE&47&94.0\%&33&66.0\%&Channel Islands English\\\hline
% \gold{\textbf{ChcE}}&30&93.8\%&28&87.5\%&Chicano English\\\hline
% CollAmE&57&83.8\%&44&64.7\%&Colloquial American English\\\hline
% CollSgE&67&89.3\%&52&69.3\%&Colloquial Singapore English (Singlish)\\\hline
% EAAVE&96&89.7\%&61&57.0\%&Earlier African American Vernacular English\\\hline
% EA&46&85.2\%&32&59.3\%&East Anglian English\\\hline
% FlkE&44&89.8\%&30&61.2\%&Falkland Islands English\\\hline
% FijiE&39&88.6\%&36&81.8\%&Acrolectal Fiji English\\\hline
% CollFijiE&95&85.6\%&68&61.3\%&Pure Fiji English (basilectal FijiE)\\\hline
% GhE&58&92.1\%&49&77.8\%&Ghanaian English\\\hline
% HKE&74&91.4\%&61&75.3\%&Hong Kong English\\\hline
% \gold{\textbf{IndE}}&90&90.0\%&82&82.0\%&Indian English\\\hline
% InSAfE&75&83.3\%&58&64.4\%&Indian South African English\\\hline
% IrE&75&81.5\%&54&58.7\%&Irish English\\\hline
% JamE&69&88.5\%&47&60.3\%&Jamaican English\\\hline
% KenE&50&90.9\%&45&81.8\%&Kenyan English\\\hline
% LibSE&86&84.3\%&58&56.9\%&Liberian Settler English\\\hline
% MalE&68&89.5\%&57&75.0\%&Malaysian English\\\hline
% MaltE&72&86.7\%&59&71.1\%&Maltese English\\\hline
% ManxE&55&83.3\%&40&60.6\%&Manx English\\\hline
% NZE&44&88.0\%&37&74.0\%&New Zealand English\\\hline
% NfldE&84&85.7\%&53&54.1\%&Newfoundland English\\\hline
% NigE&45&88.2\%&37&72.5\%&Nigerian English\\\hline
% North&77&85.6\%&47&52.2\%&English dialects in the North of England\\\hline
% O\&SE&30&81.1\%&19&51.4\%&Orkney and Shetland English\\\hline
% OzE&56&86.2\%&43&66.2\%&Ozark English\\\hline
% PakE&48&87.3\%&42&76.4\%&Pakistani English\\\hline
% PhilE&92&85.2\%&71&65.7\%&Philippine English\\\hline
% RAAVE&136&82.9\%&88&53.7\%&Rural African American Vernacular English\\\hline
% ScE&44&80.0\%&30&54.5\%&Scottish English\\\hline
% SEAmE&108&80.6\%&75&56.0\%&Southeast American enclave dialects\\\hline
% SLkE&29&82.9\%&23&65.7\%&Sri Lankan English\\\hline
% StHE&113&85.0\%&78&58.6\%&St. Helena English\\\hline
% SE&46&93.9\%&33&67.3\%&English dialects in the Southeast of England\\\hline
% SW&73&89.0\%&46&56.1\%&English dialects in the Southwest of England\\\hline
% TznE&41&93.2\%&35&79.5\%&Tanzanian English\\\hline
% TdCE&92&82.9\%&64&57.7\%&Tristan da Cunha English\\\hline
% UAAVE&118&83.7\%&79&56.0\%&Urban African American Vernacular English\\\hline
% UgE&65&86.7\%&52&69.3\%&Ugandan English\\\hline
% WelE&76&80.9\%&53&56.4\%&Welsh English\\\hline
% WhSAfE&41&83.7\%&35&71.4\%&White South African English\\\hline
% WhZimE&61&88.4\%&46&66.7\%&White Zimbabwean English\\
% \bottomrule
% \end{tabular}
% }
% \caption{\textbf{\mval{} Implemented Dialects.} They've implemented 50 English dialects as shown in this table. They list the number of implemented features (\textsc{\# Feat}), the proportion of that dialect's catalogued eWAVE features implemented (\textsc{\% Feat}), the number of validated features (\textsc{\# Val}), and the proportion of that dialect's catalogued eWAVE features validated (\textsc{\% Val}). All dialects are at or above 80\% implemented and above 51.4\% validated. Gold \gold{\textbf{ChcE}} and \gold{\textbf{IndE}} indicate that they also release a Gold CoQA dev set in Chicano and Indian English.}
% \label{tab:dialect_implementations}
% \end{table*}


% %\section{All Features}

% \begin{table*}
% \centering
% \resizebox{\textwidth}{!}{%
% \def\arraystretch{1.15}
% \begin{tabular}{rlL{75mm}L{75mm}r}
% \toprule
% {} &                     \textsc{Function} &                                            \textsc{SAE} &                                                \textsc{Transform} & \textsc{Val Acc.} \\
%  &                              &                                                    &                                                    \\
% \midrule
% \ewave{1}  &                   \texttt{she\_inanimate\_objects} &                                                         It's a good bike &                                                                               She's a good bike \\ \hline
% \ewave{2}  &                    \texttt{he\_inanimate\_objects} &              The driver's license? She wasn't allowed to renew it right? &                                    The driver's license? She wasn't allowed to renew 'im right? \\ \hline
% \ewave{3}  &                       \texttt{referential\_thing} &  Christmas dinner? I think it's better to wait until after she's had it. &                  Christmas dinner? I think it's better to wait until after she's had the thing. & 100.0\\ \hline
% \ewave{4}  &                         \texttt{pleonastic\_that} &                                                            It's raining. &                                                                                  Thass raining. \\ \hline
% \ewave{5}  &                         \texttt{em\_subj\_pronoun} &                                  This old woman, she started packing up. &                                                         This old woman, 'em started packing up. \\ \hline
% \ewave{6}  &                          \texttt{em\_obj\_pronoun} &                                                We just turned it around. &                                                                      We just turned 'im around. \\ \hline
% \ewave{7}  &                  \texttt{me\_coordinate\_subjects} &                                            Michelle and I will come too. &                                                                  Me and Michelle will come too. \\ \hline
% \ewave{8}  &              \texttt{myself\_coordinate\_subjects} &                                       My husband and I were late. &                                                         My husband and myself were late. \\ \hline
% \ewave{9}  &                      \texttt{benefactive\_dative} &                                              I have to get one of those! &                                                                  I have to get me one of those! & \gold{\textbf{ChcE}} 100.0\\ \hline
% \ewave{10} &                   \texttt{no\_gender\_distinction} &         Susan is a nurse but she does not like to put drips on patients. &                                 Susan is a nurse but he does not like to put drips on patients. & \gold{\textbf{IndE }} 97.4 \\ \hline
% \ewave{11} &                  \texttt{regularized\_reflexives} &                                                         He hurt himself. &                                                                                He hurt hisself. & 100.0 \\ \hline
% \ewave{12} &  \texttt{regularized\_reflexives\_object\_pronouns} &                                                       I'll do it myself. &                                                                              I'll do it meself. \\ \hline
% \ewave{13} &             \texttt{regularized\_reflexives\_aave} &                                              They look after themselves. &                                                                     They look after theyselves. \\ \hline
% \ewave{14} &                           \texttt{reflex\_number} &                                              We cannot change ourselves. &                                                                       We cannot change ourself. & \gold{\textbf{IndE}} 100.0 \\ \hline
% \ewave{15} &                         \texttt{absolute\_reflex} &                           and he and the bull were tuggin' and wrestlin' &                                             and himself and the bull were tuggin' and wrestlin' & \gold{\textbf{IndE}} 100.0 \\ \hline
% \ewave{16} &                         \texttt{emphatic\_reflex} &                                           They brought it by themselves. &                                                              They brought it by their own self. & \gold{\textbf{ChcE}} 100.0\\ \hline
% \ewave{18} &                                    \texttt{my\_i} &                                                                  my book &                                                                                          I book \\ \hline
% \ewave{19} &                                  \texttt{our\_we} &                                                                 our farm &                                                                                         we farm \\ \hline
% \ewave{20} &                                  \texttt{his\_he} &                                                                 his book &                                                                                         he book \\ \hline
% \ewave{21} &                              \texttt{their\_they} &                                                               their book &                                                                                       they book \\ \hline
% \ewave{22} &                                \texttt{your\_you} &                                                                your book &                                                                                        you book \\ \hline
% \ewave{23} &                              \texttt{your\_yalls} &                                                    Where are your books? &                                                                        Where are y'all's books? \\ \hline
% \ewave{24} &                                 \texttt{his\_him} &                                                                 his book &                                                                                        him book \\ \hline
% \ewave{25} &                              \texttt{their\_them} &                                                               their book &                                                                                       them book \\ \hline
% \ewave{26} &                                   \texttt{my\_me} &                                                                  my book &                                                                                         me book & 100.0\\ \hline
% \ewave{27} &                                  \texttt{our\_us} &                                                                 our book &                                                                                         us book \\ \hline
% \ewave{29} &                                   \texttt{me\_us} &                                                        Show me the town! &                                                                               Show us the town! & 100.0 \\ \hline
% \ewave{30} &                \texttt{non\_coordinated\_subj\_obj} &                                             Do you want to come with us? &                                                                    Do you want to come with we? \\ \hline
% \ewave{31} &                \texttt{non\_coordinated\_obj\_subj} &                                                   They can ride all day. &                                                                          Them can ride all day. \\ \hline
% \ewave{33} &                   \texttt{nasal\_possessive\_pron} &                                          her, his, our; hers, ours, ours &                                                           hern, hisn, ourn; hersn, oursn, ourns & 100.0\\ \hline
% \ewave{34} &                                    \texttt{yall} &                                                                      you &  y'all & \gold{\textbf{ChcE}} \gold{\textbf{IndE}} 100.0\\ \hline
% \ewave{35} &                                  \texttt{you\_ye} &                                     Sure it's no good to you in England. &                                                             Sure it's no good to ye in England. \\ \hline
% \ewave{39} &                    \texttt{plural\_interrogative} &                                                                Who came? &                                                                                   Who-all came? & 99.7\\ \hline
% \ewave{40} &               \texttt{reduplicate\_interrogative} &                                                      Who's coming today? &                                                                         Who-who's coming today? & \gold{\textbf{IndE}} 99.8 \\ \hline
% \ewave{41} &                            \texttt{anaphoric\_it} &                  Things have become more expensive than they used to be. &                                           Things have become more expensive than it used to be. & \gold{\textbf{IndE}} 100.0\\ \hline
% \ewave{42} &                     \texttt{object\_pronoun\_drop} &                                                 I got it from the store. &                                                                           I got from the store. & \gold{\textbf{IndE}} 98.1\\ \hline
% \ewave{43} &               \texttt{null\_referential\_pronouns} &             When I come back from my work I just travel back to my home. &                                      When I come back from my work just travel back to my home. & \gold{\textbf{ChcE}} \gold{\textbf{IndE}} 93.2\\ \hline
% \ewave{45} &                                 \texttt{it\_dobj} &                        As I explained to her, this is not the right way. &                                            As I explained it to her, this is not the right way. & \gold{\textbf{IndE}} 100.0\\ \hline
% \ewave{46} &                       \texttt{it\_is\_referential} &                                                    It is very nice food. &                                                                              Is very nice food. \\ \hline
% \ewave{47} &                   \texttt{it\_is\_non\_referential} &                                               Okay, it's time for lunch. &                                                                        Okay, is time for lunch. & \gold{\textbf{IndE}} 100.0\\
% \bottomrule
% \end{tabular}
% }
% \caption{Pronouns}
% \label{tab:pronouns}
% \end{table*}

% \begin{table*}
% \centering
% \resizebox{\textwidth}{!}{%
% \def\arraystretch{1.15}
% \begin{tabular}{rlL{75mm}L{75mm}r}
% \toprule
% {} &                     \textsc{Function} &                                            \textsc{SAE} &                                                \textsc{Transform} & \textsc{Val Acc.} \\
%  &                              &                                                    &                                                    \\
% \midrule
% \ewave{49} &                     \texttt{regularized\_plurals} &                                             wives, knives, lives, leaves &                                                       wifes, knifes, lifes, leafs & \gold{\textbf{IndE}} 99.6\\ \hline
% \ewave{50} &                         \texttt{plural\_preposed} &                                                           shooting birds &                                                                shooting alla bird \\ \hline
% \ewave{51} &                        \texttt{plural\_postposed} &                                                                 The boys &                                                                        Da boy dem \\ \hline
% \ewave{55} &                       \texttt{mass\_noun\_plurals} &  furniture, machinery, equipment, evidence, luggage, advice, mail, staff &  furnitures, machineries, equipments, evidences, luggages, advices, mails, staffs & \gold{\textbf{IndE}} 100.0 \\ \hline
% \ewave{56} &            \texttt{zero\_plural\_after\_quantifier} &                                               It's only five miles away. &                                                         It's only five mile away. & \gold{\textbf{ChcE}} \gold{\textbf{IndE}} 97.3 \\ \hline
% \ewave{57} &                \texttt{plural\_to\_singular\_human} &                          The three girls there don't want to talk to us. &                                    The three girl there don't want to talk to us.& \gold{\textbf{IndE}} 100.0 \\ \hline
% \ewave{58} &                             \texttt{zero\_plural} &                                              Some apartments are bigger. &                                                        Some apartment are bigger.& \gold{\textbf{IndE}} 100.0 \\ \hline
% \ewave{59} &                      \texttt{double\_determiners} &                             This common problem of ours is very serious. &                                          This our common problem is very serious.& \gold{\textbf{IndE}} 100.0 \\ \hline
% \ewave{60} &        \texttt{definite\_for\_indefinite\_articles} &                                                   She's got a toothache. &                                                           She's got the toothache & \gold{\textbf{IndE}} 99.6\\ \hline
% \ewave{61} &        \texttt{indefinite\_for\_definite\_articles} &                                     The moon was very bright last night. &                                                A moon was very bright last night. & \gold{\textbf{IndE}} 100.0\\ \hline
% \ewave{62} &                     \texttt{remove\_det\_definite} &                                                      He's in the office. &                                                                   He's in office. & \gold{\textbf{IndE}} 100.0\\ \hline
% \ewave{63} &                   \texttt{remove\_det\_indefinite} &                                                Can I get a better grade? &                                                           Can I get better grade? & \gold{\textbf{IndE}} 99.0\\ \hline
% \ewave{64} &                       \texttt{definite\_abstract} &                                             I stayed on until Christmas. &                                                  I stayed on until the Christmas. & \gold{\textbf{IndE}} 100.0 \\ \hline
% \ewave{65} &                     \texttt{indefinite\_for\_zero} &                                           We received good news at last. &                                                  We received a good news at last. \\ \hline
% \ewave{66} &                               \texttt{indef\_one} &                                         What happened? Oh, a dog bit me. &                                                What happened? Oh, one dog bit me. & \gold{\textbf{IndE}} 100.0 \\ \hline
% \ewave{67} &     \texttt{demonstrative\_for\_definite\_articles} &                  They have two children. The elder girl is 19 years old. &                          They have two children. That elder girl is 19 years old. & \gold{\textbf{IndE}} 99.1\\ \hline
% \ewave{68} &                              \texttt{those\_them} &                                I don't have any of those qualifications. &                                          I don't have any of them qualifications. \\ \hline
% \ewave{70} &          \texttt{proximal\_distal\_demonstratives} &         this book that is right here vs. those books that are over there &                                               this here book vs. them there books & \gold{\textbf{ChcE}} 92.9\\ \hline
% \ewave{71} &                 \texttt{demonstrative\_no\_number} &                                     These books are useful for my study. &                                               This books are useful for my study. & \gold{\textbf{IndE}} 98.8\\ \hline
% \ewave{73} &                 \texttt{existential\_possessives} &                                                            I have a son. &                                                                     Son is there. \\ \hline
% \ewave{74} &                    \texttt{possessives\_for\_post} &                                               This is my mother's house. &                                                  This is the house for my mother. \\ \hline
% \ewave{75} &                     \texttt{possessives\_for\_pre} &                                Long time ago he was my sister's husband. &                                           Long time he was for my sister husband. \\ \hline
% \ewave{76} &                      \texttt{possessives\_belong} &                                                       the woman's friend &                                                               woman belong friend \\ \hline
% \ewave{77} &                           \texttt{null\_genitive} &                                                         my cousin's bike &                                                                    my cousin bike & \gold{\textbf{IndE}} 100.0\\ \hline
% \ewave{78} &  \texttt{double\_comparative, double\_superlative} &                                        That is so much easier to follow. &                                            That is so much more easier to follow. & \gold{\textbf{IndE}} 100.0\\ \hline
% \ewave{79} &                   \texttt{synthetic\_superlative} &                                       He is the most regular guy I know. &                                                  He is the regularest guy I know. & \gold{\textbf{IndE}} 100.0\\ \hline
% \ewave{80} &                    \texttt{analytic\_superlative} &                                             one of the prettiest sunsets &                                                    one of the most pretty sunsets & \gold{\textbf{IndE}} 100.0\\ \hline
% \ewave{81} &                               \texttt{more\_much} &                            The situation is more serious than I thought. &                                     The situation is much serious than I thought. & \gold{\textbf{IndE}} 100.0\\ \hline
% \ewave{82} &                       \texttt{comparative\_as\_to} &                                           She is bigger than her sister. &                                                      She is bigger as her sister. \\ \hline
% \ewave{84} &                        \texttt{comparative\_than} &                                 They like football more than basketball. &                                               They like football than basketball. \\ \hline
% \ewave{85} &                    \texttt{comparative\_more\_and} &                                      He has more clothes than all of us. &                                                He has more clothes and all of us. \\ \hline
% \ewave{86} &                             \texttt{zero\_degree} &           He is one of the most radical students that you can ever find. &                         He is one of the radical students that you can ever find. & \gold{\textbf{IndE}} 100.0\\ \hline
% \ewave{87} &                             \texttt{adj\_postfix} &                                     A big and fresh fish is my favorite. &                                              A fish big and fresh is my favorite. \\
% \bottomrule
% \end{tabular}
% }
% \caption{Noun Phrases}
% \label{tab:nounphrases}
% \end{table*}

% \begin{table*}
% \centering
% \resizebox{\textwidth}{!}{%
% \def\arraystretch{1.15}
% \begin{tabular}{rlL{75mm}L{75mm}r}
% \toprule
% {} &                     \textsc{Function} &                                            \textsc{SAE} &                                                \textsc{Transform} & \textsc{Val Acc.} \\
%  &                              &                                                    &                                                    \\
% \midrule
% \ewave{88}  &                      \texttt{progressives} &                                    I like her hair style right now. &                                            I am liking her hair style. & \gold{\textbf{IndE}} 99.4\\ \hline
% \ewave{95}  &                    \texttt{standing\_stood} &                                      He was standing on the corner. &                                            He was stood on the corner. \\ \hline
% \ewave{96}  &  \texttt{that\_resultative\_past\_participle} &                         There is a car that broke down on the road. &                                There is a car broken down on the road. & 95.5 \\ \hline
% \ewave{97}  &             \texttt{medial\_object\_perfect} &                                            He has written a letter. &                                               He has a letter written. \\ \hline
% \ewave{98}  &                     \texttt{after\_perfect} &                                         She has just sold the boat. &                                          She's after selling the boat. \\ \hline
% \ewave{99}  &   \texttt{simple\_past\_for\_present\_perfect} &                               I've eaten the food. So can I go now? &                                       I ate the food. So can I go now? & \gold{\textbf{ChcE}} 94.7 \\ \hline
% \ewave{100} &          \texttt{present\_perfect\_for\_past} &                                            We were there last year. &                                            We've been there last year. & \gold{\textbf{IndE}} 99.9\\ \hline
% \ewave{101} &           \texttt{present\_for\_exp\_perfect} &                               I've known her since she was a child. &                                      I know her since she was a child. & \gold{\textbf{IndE}} 100.0\\ \hline
% \ewave{102} &                        \texttt{be\_perfect} &                                       They haven't left school yet. &                                           They're not left school yet. \\ \hline
% \ewave{103} &                   \texttt{do\_tense\_marker} &                                   I knew some things weren't right. &                                  I did know some things weren't right. \\ \hline
% \ewave{104} &                   \texttt{completive\_done} &                                     Sharon has read the whole book. &                                       Sharon done read the whole book. \\ \hline
% \ewave{105} &              \texttt{completive\_have\_done} &                                             He has talked about me. &                                           He has done talked about me. \\ \hline
% \ewave{106} &                  \texttt{irrealis\_be\_done} &  If you love your enemies, they will eat you alive in this society. &  If you love your enemies, they be done eat you alive in this society. & 100.0\\ \hline
% \ewave{107} &                      \texttt{perfect\_slam} &                                                                 I have already told you not to mess up &                                                                    I slam told you not to mess up. \\ \hline
% \ewave{108} &              \texttt{present\_perfect\_ever} &                                              I have seen the movie. &                                                  I ever see the movie. \\ \hline
% \ewave{109} &                   \texttt{perfect\_already} &                                               Have you eaten lunch? &                                                   Did you eat already? \\ \hline
% \ewave{110} &                 \texttt{completive\_finish} &                                                       I have eaten. &                                                          I finish eat. \\ \hline
% \ewave{111} &                         \texttt{past\_been} &                                                         I told you. &                                                       I been told you. \\ \hline
% \ewave{112} &                      \texttt{bare\_perfect} &                       We had caught the fish when the big wave hit. &                           We had catch the fish when the big wave hit. \\ \hline
% \ewave{114} &                    \texttt{future\_sub\_gon} &                                               He will come with us. &                                                  He gon' come with us. \\ \hline
% \ewave{115} &                  \texttt{volition\_changes} &                                                     You want to go. &                                                           You waan go. \\ \hline
% \ewave{116} &                       \texttt{come\_future} &                                       I am about to cook your meal. &                                         I am coming to cook your meal. \\ \hline
% \ewave{117} &        \texttt{present\_for\_neutral\_future} &       Next week, I will be leaving the States and going to Liberia. &                   Next week, I leaving the States, I going to Liberia. & \gold{\textbf{IndE}} 100.0\\ \hline
% \ewave{118} &                          \texttt{is\_am\_1s} &                                                 I am going to town. &                                                     I's going to town. \\ \hline
% \ewave{119} &                        \texttt{will\_would} &                                           I will meet him tomorrow. &                                             I would meet him tomorrow.& \gold{\textbf{IndE}} 100.0 \\ \hline
% \ewave{120} &                          \texttt{if\_would} &                                  If I were you I would go home now. &                                 If I would be you I would go home now. \\
% \bottomrule
% \end{tabular}
% }
% \caption{Tense and Aspect}
% \label{tab:tenseaspect}
% \end{table*}

% \begin{table*}
% \centering
% \resizebox{\textwidth}{!}{%
% \def\arraystretch{1.15}
% \begin{tabular}{rlL{75mm}L{75mm}r}
% \toprule
% {} &                     \textsc{Function} &                                            \textsc{SAE} &                                                \textsc{Transform} & \textsc{Val Acc.}\\
%  &                              &                                                    &                                                    \\
% \midrule
% \ewave{121} &               \texttt{double\_modals} &            We could do that. &                 We might could do that. & \gold{\textbf{ChcE  }} 91.8\\ \hline
% \ewave{123} &              \texttt{present\_modals} &  I wish I could get the job. &               I wish I can get the job. & \gold{\textbf{IndE}} 100.0\\ \hline
% \ewave{126} &  \texttt{finna\_future, fixin\_future} &      They're about to leave. &  They're fixin to leave town. & \gold{\textbf{ChcE  }} 92.3\\
% \bottomrule
% \end{tabular}
% }
% \caption{Mood}
% \label{tab:mood}
% \end{table*}

% \begin{table*}
% \centering
% \resizebox{\textwidth}{!}{%
% \def\arraystretch{1.15}
% \begin{tabular}{rlL{75mm}L{75mm}r}
% \toprule
% {} &                     \textsc{Function} &                                            \textsc{SAE} &                                                \textsc{Transform} & \textsc{Val Acc.}\\
%  &                              &                                                    &                                                    \\
% \midrule
% \ewave{128} &    \texttt{regularized\_past\_tense} &                     He caught the ball. &                      He catched the ball. & \gold{\textbf{ChcE}} \gold{\textbf{IndE}} 92.7\\ \hline
% \ewave{129} &           \texttt{bare\_past\_tense} &                They came and joined us. &                  They come and joined us. \\ \hline
% \ewave{130} &  \texttt{past\_for\_past\_participle} &                            He had gone. &                              He had went. & \gold{\textbf{ChcE}} 92.9 \\ \hline
% \ewave{131} &     \texttt{participle\_past\_tense} &                               I saw it. &                                I seen it. & \gold{\textbf{IndE}} 100.0 \\ \hline
% \ewave{132} &           \texttt{bare\_past\_tense} &  Here are things you ordered yesterday. &      Here are things you order yesterday. & \gold{\textbf{ChcE}} \gold{\textbf{IndE}} 87.7\\ \hline
% \ewave{133} &               \texttt{double\_past} &          They didn't make it this time. &            They didn't made it this time. & \gold{\textbf{IndE}} 99.5\\ \hline
% \ewave{134} &                     \texttt{a\_ing} &                    Where are you going? &                     Where are you a-goin? & 100.0\\ \hline
% \ewave{135} &              \texttt{a\_participle} &              You've killed your mother. &              You've a-killed your mother. \\ \hline
% \ewave{143} &         \texttt{transitive\_suffix} &                   You can see the fish. &                     You can see 'im fish. \\ \hline
% \ewave{145} &                \texttt{got\_gotten} &   I hope you've got your topic already. &  I hope you've gotten your topic already. & 100.0\\ \hline
% \ewave{146} &         \texttt{verbal\_ing\_suffix} &                        I can drive now. &                        I can driving now. & \gold{\textbf{IndE}} 100.0 \\ \hline
% \ewave{147} &      \texttt{conditional\_were\_was} &                           If I were you &                              If I was you \\ \hline
% \ewave{148} &          \texttt{serial\_verb\_give} &                  I bought rice for you. &                      I buy rice give you. \\ \hline
% \ewave{149} &            \texttt{serial\_verb\_go} &         Grandfather sends us to school. &            Grandfather send us go school. & 100.0\\ \hline
% \ewave{150} &                 \texttt{here\_come} &                    Bring the book here. &                 Take the book bring come. \\ \hline
% \ewave{153} &              \texttt{give\_passive} &            John was scolded by his boss &                 John give his boss scold. \\
% \bottomrule
% \end{tabular}
% }
% \caption{Verb Morphology}
% \label{tab:verbmorphology}
% \end{table*}

% \begin{table*}
% \centering
% \resizebox{\textwidth}{!}{%
% \def\arraystretch{1.15}
% \begin{tabular}{rlL{75mm}L{75mm}r}
% \toprule
% {} &                     \textsc{Function} &                                            \textsc{SAE} &                                                \textsc{Transform} & \textsc{Val Acc.}\\
%  &                              &                                                    &                                                    \\
% \midrule
% \ewave{154} &            \texttt{negative\_concord} &                           I don't want any help. &                   I don't want no help. & \gold{\textbf{ChcE}} \gold{\textbf{IndE}} 92.9\\ \hline
% \ewave{155} &                     \texttt{aint\_be} &                                 That isn't fair. &                        That ain't fair. & \gold{\textbf{ChcE}} 81.8\\ \hline
% \ewave{156} &                   \texttt{aint\_have} &                          I hadn't seen them yet. &                  I ain't seen them yet. \\ \hline
% \ewave{157} &            \texttt{aint\_before\_main} &                    something I didn't know about &            something I ain't know about \\ \hline
% \ewave{158} &                        \texttt{dont} &                He doesn't always tell the truth. &         He don't always tell the truth. \\ \hline
% \ewave{159} &               \texttt{never\_negator} &                                  He didn't come. &                          He never came. & 100.0 \\ \hline
% \ewave{160} &        \texttt{no\_preverbal\_negator} &                I don't want any job or anything. &          I no want any job or anything. \\ \hline
% \ewave{161} &       \texttt{not\_preverbal\_negator} &        The baby didn't eat food and cried a lot. &  The baby not ate food and cried a lot. \\ \hline
% \ewave{162} &            \texttt{nomo\_existential} &       There is not any food in the refrigerator. &       No more food in the refrigerator. \\ \hline
% \ewave{163} &                \texttt{wasnt\_werent} &                  John was there, but Mike wasn't &        John was there, but Mike weren't \\ \hline
% \ewave{164} &          \texttt{invariant\_tag\_amnt} &  I believe I am older than you. Is that correct? &           I am older than you, amn't I? \\ \hline
% \ewave{165} &   \texttt{invariant\_tag\_non\_concord} &          I believe you are ill. Is that correct? &                  You are ill, isn't it? & \gold{\textbf{IndE}} 99.1\\ \hline
% \ewave{166} &    \texttt{invariant\_tag\_can\_or\_not} &                                   Can I go home? &          I want to go home, can or not? \\ \hline
% \ewave{167} &  \texttt{invariant\_tag\_fronted\_isnt} &                      I can go there now can't I? &              Isn't, I can go there now? \\
% \bottomrule
% \end{tabular}
% }
% \caption{Negation}
% \label{tab:negation}
% \end{table*}

% \begin{table*}
% \centering
% \resizebox{\textwidth}{!}{%
% \def\arraystretch{1.15}
% \begin{tabular}{rlL{75mm}L{75mm}r}
% \toprule
% {} &                     \textsc{Function} &                                            \textsc{SAE} &                                                \textsc{Transform} & \textsc{Val Acc.} \\
%  &                              &                                                    &                                                    \\
% \midrule
% \ewave{170} &                   \texttt{uninflect} &                      He speaks English. &                                                            He speak English. & \gold{\textbf{ChcE}} \gold{\textbf{IndE}} 94.9\\ \hline
% \ewave{171} &  \texttt{generalized\_third\_person\_s} &           Every Sunday we go to church. &                                              Every Sunday we goes to church. \\ \hline
% \ewave{172} &           \texttt{existential\_there} &  There are two men waiting in the hall. &                                         There's two men waiting in the hall. & \gold{\textbf{ChcE}} \gold{\textbf{IndE}} 90.0\\ \hline
% \ewave{173} &              \texttt{existential\_it} &        There's some milk in the fridge. &                                                It's some milk in the fridge. & \gold{\textbf{ChcE}} 87.5 \\ \hline
% \ewave{174} &     \texttt{drop\_aux\_be\_progressive} &       You are always thinking about it. &                                                You always thinking about it. & \gold{\textbf{IndE}} 100.0\\ \hline
% \ewave{175} &           \texttt{drop\_aux\_be\_gonna} &       He is gonna go home and watch TV. &                                               He gonna go home and watch TV. & \gold{\textbf{ChcE}} \gold{\textbf{IndE}} 83.3 \\ \hline
% \ewave{176} &           \texttt{drop\_copula\_be\_NP} &                   He is a good teacher. &                                                           He a good teacher. \\ \hline
% \ewave{177} &           \texttt{drop\_copula\_be\_AP} &                           She is smart. &                                                                   She smart. \\ \hline
% \ewave{178} &     \texttt{drop\_copula\_be\_locative} &                         She is at home. &                                                                 She at home. \\ \hline
% \ewave{179} &               \texttt{drop\_aux\_have} &                  I have seen it before. &                                                            I seen it before. & \gold{\textbf{IndE}} 100.0\\ \hline
% \ewave{180} &                    \texttt{were\_was} &     You were hungry but he was thirsty. &  You was hungry but he was thirsty. OR: You were hungry but he were thirsty. \\
% \bottomrule
% \end{tabular}
% }
% \caption{Agreement}
% \label{tab:agreement}
% \end{table*}

% \begin{table*}
% \centering
% \resizebox{\textwidth}{!}{%
% \def\arraystretch{1.15}
% \begin{tabular}{rlL{75mm}L{75mm}r}
% \toprule
% {} &                     \textsc{Function} &                                            \textsc{SAE} &                                                \textsc{Transform} & \textsc{Val Acc.}\\
%  &                              &                                                    &                                                    \\
% \midrule
% \ewave{186} &                   \texttt{who\_which} &                                                                           He's the man who looks after the cows. &                                                                 He's the man which looks after the cows. \\ \hline
% \ewave{187} &                      \texttt{who\_as} &                                                                                       The man who was just here. &                                                                                The man as was just here. \\ \hline
% \ewave{188} &                      \texttt{who\_at} &                                                                            This is the man who painted my house. &                                                                     This is the man at painted my house. \\ \hline
% \ewave{189} &           \texttt{relativizer\_where} &  My father was one of the founders of the Underground Railroad, which helped the slaves to run away to the North &  My father was one o de founders o' de Underground Railroad where help de slaves to run way to de North. \\ \hline
% \ewave{190} &                    \texttt{who\_what} &                                                                            This is the man who painted my house. &                                                                   This is the man what painted my house. \\ \hline
% \ewave{191} &        \texttt{relativizer\_doubling} &                                                            But these, these little fellahs who had stayed before &                                              But these, these little fellahs that which had stayed befo' & \gold{\textbf{IndE}} 100.0\\ \hline
% \ewave{192} &  \texttt{analytic\_whose\_relativizer} &                                                                             This is the man whose wife has died. &                      This is the man that his wife has died. OR: This is the man what his wife has died. \\ \hline
% \ewave{193} &                  \texttt{null\_relcl} &                                                                             The man who lives there is friendly. &                                                                         The man lives there is friendly. & \gold{\textbf{ChcE}} \gold{\textbf{IndE}} 88.7\\ \hline
% \ewave{194} &             \texttt{shadow\_pronouns} &                                                                     This is the house which I painted yesterday. &                                                          This is the house which I painted it yesterday. & \gold{\textbf{IndE}} 100.0 \\ \hline
% \ewave{195} &             \texttt{one\_relativizer} &                                                              The cake that John buys is always very nice to eat. &                                                           The cake John buy one always very nice to eat. \\ \hline
% \ewave{196} &   \texttt{correlative\_constructions} &                                                                               The ones I made are the good ones. &                                                                        The one I made, that one is good. \\ \hline
% \ewave{197} &               \texttt{linking\_relcl} &                          Unless you are going to get 88, but some universities are not going to give those marks &                 Unless you are going to get 88 which some universities are not going to give those marks \\ \hline
% \ewave{198} &        \texttt{preposition\_chopping} &                                                      You remember the swing that we all used to sit together on? &                                                 You remember the swing that we all used to sit together?& \gold{\textbf{IndE}} 100.0 \\ \hline
% \ewave{199} &            \texttt{reduced\_relative} &                                                                       There is nothing like food cooked by Amma! &                                                                  There is nothing like Amma cooked food! \\
% \bottomrule
% \end{tabular}
% }
% \caption{Relativization}
% \label{tab:relativization}
% \end{table*}

% \begin{table*}
% \centering
% \resizebox{\textwidth}{!}{%
% \def\arraystretch{1.15}
% \begin{tabular}{rlL{75mm}L{75mm}r}
% \toprule
% {} &                     \textsc{Function} &                                            \textsc{SAE} &                                                \textsc{Transform} & \textsc{Val Acc.} \\
%  &                              &                                                    &                                                    \\
% \midrule
% \ewave{200} &          \texttt{say\_complementizer} &                            We hear that you were gone to the city. &                                                                 We hear say you gone to the city. \\ \hline
% \ewave{201} &          \texttt{for\_complementizer} &          You mean your mother allows you to bring over boyfriends? &                                        You mean your mother allows you for bring over boyfriends? \\ \hline
% \ewave{202} &               \texttt{for\_to\_pupose} &  We always had gutters in the winter time to drain the water away. &                             We always had gutters in the winter time for to drain the water away. \\ \hline
% \ewave{203} &                      \texttt{for\_to} &                        He had the privilege to turn on the lights. &  He had the privilege for to turn on the lights. OR: He had the privilege for turn on the lights. & 100.0\\ \hline
% \ewave{204} &            \texttt{what\_comparative} &                                             I'm taller than he is. &                                                                       I'm taller than what he is. & \gold{\textbf{IndE}} 100.0\\ \hline
% \ewave{205} &             \texttt{existential\_got} &                                    There's no water in the toilet. &                                                                       Got no water in the toilet. & 100.0\\ \hline
% \ewave{206} &        \texttt{existential\_you\_have} &         There are some people who don't give a damn about animals. &                                        You have some people they don't give a damn about animals. & \gold{\textbf{IndE}} 100.0\\ \hline
% \ewave{207} &  \texttt{that\_infinitival\_subclause} &                                       He wanted me to go with him. &                                                              He wanted that I should go with him. & \gold{\textbf{IndE}} 100.0\\ \hline
% \ewave{208} &                 \texttt{drop\_inf\_to} &                                     They were allowed to call her. &                                                                       They were allowed call her. & 100.0\\ \hline
% \ewave{209} &               \texttt{to\_infinitive} &                                                  He made me do it. &                                                                              He made me to do it. & \gold{\textbf{IndE}} 100.0\\ \hline
% \ewave{210} &                  \texttt{bare\_ccomp} &              When mistress started whooping her, she sat her down. &                                                When mistress started whoop her, she sat her down. \\
% \bottomrule
% \end{tabular}
% }
% \caption{Complementation}
% \label{tab:complementation}
% \end{table*}

% \begin{table*}
% \centering
% \resizebox{\textwidth}{!}{%
% \def\arraystretch{1.15}
% \begin{tabular}{rlL{75mm}L{75mm}r}
% \toprule
% {} &                     \textsc{Function} &                                            \textsc{SAE} &                                                \textsc{Transform} & \textsc{Val Acc.}\\
%  &                              &                                                    &                                                    \\
% \midrule
% \ewave{211} &      \texttt{clause\_final\_though\_but} &                          There's nothing wrong with this box though. &                               There's nothing wrong with this box, but. \\ \hline
% \ewave{212} &      \texttt{clause\_final\_really\_but} &                           I don't know what else she can do, really. &                                 I don't know what else she can do, but. \\ \hline
% \ewave{213} &          \texttt{chaining\_main\_verbs} &                        If you stay longer, they have to charge more. &                                  Stay longer, they have to over-charge. \\ \hline
% \ewave{214} &    \texttt{corr\_conjunction\_doubling} &  Despite being instructed on what to do, he still made some misakes. &  Despite being instructed on what to do still yet he made some misakes.& \gold{\textbf{IndE}} 100.0 \\ \hline
% \ewave{215} &  \texttt{subord\_conjunction\_doubling} &                      Although you are smart, you are not appreciated &                     Although you are smart, but you are not appreciated \\
% \bottomrule
% \end{tabular}
% }
% \caption{Adverbial Subordination}
% \label{tab:adverbialsubordination}
% \end{table*}

% \begin{table*}
% \centering
% \resizebox{\textwidth}{!}{%
% \def\arraystretch{1.15}
% \begin{tabular}{rlL{75mm}L{75mm}r}
% \toprule
% {} &                     \textsc{Function} &                                            \textsc{SAE} &                                                \textsc{Transform} & \textsc{Val Acc.}\\
%  &                              &                                                    &                                                    \\
% \midrule
% \ewave{216} &   \texttt{null\_prepositions} &                             I'm going to town. &                               I'm going town. & \gold{\textbf{IndE}} 99.7\\ \hline
% \ewave{220} &  \texttt{degree\_adj\_for\_adv} &                    That's really nice and cold &                     That's real nice and cold &\gold{\textbf{ChcE}} \gold{\textbf{IndE}} 99.4\\ \hline
% \ewave{221} &    \texttt{flat\_adj\_for\_adv} &                          She speaks so softly. &                           She speaks so soft. & \gold{\textbf{ChcE}} \gold{\textbf{IndE}} 86.7 \\ \hline
% \ewave{222} &             \texttt{too\_sub} &  They are very nice. We had a good time there. &  They are too nice. We had a good time there. \\
% \bottomrule
% \end{tabular}
% }
% \caption{Adverbs and Prepositions}
% \label{tab:adverbsprepositions}
% \end{table*}

% \begin{table*}
% \centering
% \resizebox{\textwidth}{!}{%
% \def\arraystretch{1.15}
% \begin{tabular}{rlL{75mm}L{75mm}r}
% \toprule
% {} &                     \textsc{Function} &                                            \textsc{SAE} &                                                \textsc{Transform} & \textsc{Val Acc.} \\
%  &                              &                                                    &                                                    \\
% \midrule
% \ewave{223} &                        \texttt{clefting} &  A lot of them are looking for more land. &  It's looking for more land a lot of them are. & 100.0\\ \hline
% \ewave{224} &                   \texttt{fronting\_pobj} &           I drive to town every Saturday. &                To town every Saturday I drive. & \gold{\textbf{IndE}} 99.5\\ \hline
% \ewave{226} &              \texttt{negative\_inversion} &                         Nobody showed up. &                         Didn't nobody show up. & 100.0\\ \hline
% \ewave{227} &      \texttt{inverted\_indirect\_question} &   I'm wondering what you are going to do. &        I'm wondering what are you going to do. & \gold{\textbf{ChcE}} \gold{\textbf{IndE}} 91.2\\ \hline
% \ewave{228} &                     \texttt{drop\_aux\_wh} &                       When is she coming? &                               When she coming? & \gold{\textbf{IndE}} 99.8\\ \hline
% \ewave{229} &                     \texttt{drop\_aux\_yn} &                     Do you get the point? &                             You get the point? & \gold{\textbf{IndE}} 99.9\\ \hline
% \ewave{230} &              \texttt{doubly\_filled\_comp} &                             Who ate what? &                            What who has eaten? \\ \hline
% \ewave{231} &  \texttt{superlative\_before\_matrix\_head} &          The thing I like most is apples. &               The most thing I like is apples. \\ \hline
% \ewave{232} &                \texttt{double\_obj\_order} &                 She would teach it to us. &                             She'd teach us it. & \gold{\textbf{IndE}} 100.0\\ \hline
% \ewave{234} &             \texttt{acomp\_focusing\_like} &                      It was really cheap. &                      It was like really cheap. & \gold{\textbf{ChcE}} \gold{\textbf{IndE}} 91.2\\ \hline
% \ewave{235} &                  \texttt{quotative\_like} &              And my friend said "No way!" &               And my friend was like "No way!" \\
% \bottomrule
% \end{tabular}
% }
% \caption{Discourse and Word Order}
% \label{tab:discoursewordorder}
% \end{table*}
